Bottom-up rewriting for words and terms

For the whole class of linear term rewriting systems, we define \emph{bottom-up rewriting} which is a restriction of the usual notion of rewriting. We show that bottom-up rewriting effectively inverse-preserves recognizability and analyze the complexity of the underlying construction. The Bottom-Up class (BU) is, by definition, the set of linear systems for which every derivation can be replaced by a bottom-up derivation. Membership to BU turns out to be undecidable, we are thus lead to define more restricted classes: the classes SBU(k), k in N of Strongly Bottom-Up(k) systems for which we show that membership is decidable. We define the class of Strongly Bottom-Up systems by SBU = U_{k in \} SBU(k). We give a polynomial sufficient condition for a system to be in $\SBU$. The class SBU contains (strictly) several classes of systems which were already known to inverse preserve recognizability: the inverse left-basic semi-Thue systems (viewed as unary term rewriting systems), the linear growing term rewriting systems, the inverse Linear-Finite-Path-Ordering systems.

==> Makefile <==
NAME = bottom-up
SHORT = short
TEXFILES=$(NAME).tex $(shell ./tex-dependencies $(NAME).tex)
PSTEX_T=$(shell ./strip-dependence inputfig $(TEXFILES))
#VERBATIM=$(shell ./strip-dependence verbatimtabinput $(TEXFILES))
PSTEX=$(subst .pstex_t,.pstex,$(PSTEX_T))

.SUFFIXES:
.SUFFIXES: .fig .ps .dvi .tex

all : $(NAME).ps # $(SHORT).ps

$(NAME).dvi: $(TEXFILES) $(PSTEX_T)  $(NAME).bbl #$(VERBATIM)
	echo '\def\courte{0}' > VERSION
	echo '\def\longue{1}' >> VERSION
	latex $<
	latex $<

$(NAME).ps: $(NAME).dvi $(PSTEX)
	dvips $< -o

$(NAME).bbl: references.bib
	latex $(NAME)
	bibtex $(NAME)
	latex $(NAME)

$(SHORT).dvi: $(TEXFILES) $(PSTEX_T) $(NAME).bbl #$(VERBATIM)
	echo '\def\courte{1}' > VERSION
	echo '\def\longue{2}' >> VERSION
	cp $(NAME).tex $(SHORT).tex
	latex $(SHORT)
	latex $(SHORT)
#	-rm -f $<.tex

%.pstex: %.fig
	fig2dev -Lpstex -m 0.75  $< $@

%.pstex_t: %.fig %.pstex
	fig2dev -Lpstex_t -m 0.75 -p $(basename $<).pstex $< $@

.ps.pdf :
	ps2pdf $*.ps

.dvi.ps :
	dvips $*.dvi -o 

.fig.ps :
	fig2dev -Lps -Pc $*.fig > $*.ps

.tex.dvi:
	latex $*

see:
	gv $(NAME).ps

web:
	cp $(NAME).ps ~/public_html/

clean:
	-rm -f *.aux *.log *. *~ *.blg 

veryclean:
	make clean
	-rm -f  $(NAME).bbl *.{pstex,pstex_t} $(NAME).toc *.fig.bak

spotless:
	make veryclean
	-rm -f $(NAME).{dvi,ps}


==> VERSION <==
\def\def\longue{1}


==> recognizability.tex <==

Given a linear systems $\RR$ and a set of terms $T$ recognized by
and automaton $\AA_T$, we will construct an automaton
recognizing the set of terms which bottom-up rewrites to
a term in $T$.

\subsection{Preliminary constructions}
Let $(\RR,\FF)$ be a linear systems. 
Let $\FF_\AA$ be a signature compatible with $\FF$ (\emph{i.e} symbols with identical
names have the same arity).
Let $T \subseteq \TT(\FF_\AA)$ be a recognizable set of terms
and $\AA_T = (\FF_\AA, Q_\AA, Q_\AA^f, \sysa)$ an automaton
recognizing $T$. We assume without loss of generality that all states of
$\AA_T$ are accessible.

Throughout the whole section, we will illustrate the constructions with the 
linear system 
$(\RR,\FF)$ with $\FF = \{ a^{(0)}, b^{(0)}, g^{(2)} \}$
and 
\[
\RR = \left\{
\begin{array}{l@{~\to~}l}
g(g(x,b),a) & g(x,b)
\end{array}
\right.
\]
and the automaton
$\AA = (\FF_\AA, Q_\AA, Q_\AA^f, \sysa)$ with 
$\FF_\AA = \{ a^{(0)}, b^{(0)}, h^{(2)}, g^{(2)} \}$,
$Q_\AA = \{ q_a, q_b, q^f \}$, $Q_\AA^f = \{ q^f \}$ and
\[
\sysa = \left\{ 
\begin{array}{l@{~\to~}l}
a              & q_{a}\\
b              & q_{b}\\
g(q_a,q_b) & q^f\\
\end{array}
\right.
\]

It is easy to see that $\TT = \{ g(a,b) \}$.
and that $(\to_\RR^*)[L(\AA_\TT)]$ contains $g(a,b)$
and the terms of the form
$g(g(\ldots g(g(a,b),a) \ldots, a),a)$.

Using Definition~\ref{d-sysci}, we obtain
\[
\sysa^\circ = \left\{ 
\begin{array}{l@{~\to~}l}
a^\circ          & q_a\\
b^\circ          & q_b\\
g^\circ(q_a,q_b) & q^f\\
\end{array}
\right.
\]

\subsection{Step 1}
\label{ss-step1}
We consider that linear terms are equal if they can be made
syntactically equal by variable renaming. 
%% For our examples, we will rename the variables from left to right,
%% using the ordered variables  $\VV = \{ x, x_1, x_2, \ldots \}$.
%% For instance the term $h(z,b)$ will be renamed $h(x,b)$.

Let $\SS_\RR = 
\{ (\sto{l}{u})\theta \mid l \to r \in \RR, u \in \Pos(l), 
\theta:\Var(\sto{l}{u}) \cap \Var(r) \to Q_\AA \}$.

We construct the term automaton $\BB(\RR) = (\GG, Q_\BB, \varnothing, \sys_\BB)$
with $\GG = \FF \cup \FF_\AA$,
with $Q_\BB = \{ \state{t} \mid t \in \SS_\RR \}$
and
$\sys_\BB$ consisting of \emph{matching rules}
$g(\state{t_1\theta}, \ldots, \state{t_n\theta}) \to \state{g(t_1,\ldots,t_m)\theta}$
for every $\state{g(t_1,\ldots,t_m)\theta} = \state{(\sto{l}{u})\theta} \in Q_\BB$
and in the case where $\state{x} \in Q_\BB$ 
\emph{propagation} rules $f(\state{x}, \dots, \state{x}) \to \state{x}$ for every $f \in \GG$.

For our example we obtain
\[
\GG = \{  a^{(0)}, b^{(0)},h^{(2)}, g^{(2)}\}
\]
\[
\SS_\RR = \{ q_a, q_b, q^f, 
             b, 
             g(q_{a},b), g(q_b,b), g(q^f,b),
             g(g(q_a,b),a),g(g(q_b,b),a),
             g(g(q^f,b),a) \}
\]
\[
Q_\BB = \left\{ 
\begin{array}{l}
\state{q_{a}},\state{q_b}, \state{q^f}, \state{b}, \\
\state{g(q_{a},b)}, 
\state{g(q_b,b)}, 
\state{g(q^f,b)},\\
\state{g(g(q_a,b),a)},
\state{g(g(q_b,b),a)},
\state{g(g(q^f,b),a)}
\end{array}
\right\}
\]

$\sysb$ contains the following matching rules.
\[
\sysb =
\left\{
\begin{array}{l@{~\to~}l}
b                                               & \state{b}\\
g(\state{q_a},\state{b})                    & \state{g(q_{a},b)}\\
g(\state{q_b},\state{b})         & \state{g(q_b,b)}\\
g(\state{q^f},\state{b})                      & \state{g(q^f,b)}\\
g(\state{g(q_a,b)},\state{a})           & \state{g(g(q_a,b),a)}\\
g(\state{g(q_b,b)},\state{a})& \state{g(g(q_b,b),a)}\\
g(\state{g(q^f,b)},\state{a})             & \state{g(g(q^f,b),a)}\\
\end{array}
\right.
\]
There are no propagation rules because the only variable
in the left-handside appears also in the right-handside so we have no 
state $\state{x}$).

\subsection{Step 2}
\label{ss-step2}
We define the set $\sysi$ of \emph{interaction} rules between states of $Q_\AA$ and states of $Q_\BB$
as  $\sysi = \{ q \to \state{q} \mid \state{q} \in Q_\BB, q \in Q_\AA \}$.
\[
\sysi = \left\{
\begin{array}{l@{~\to~}l}
q_{a} & \state{q_{a}}\\
q_b & \state{q_b}\\
q^f & \state{q^f}\\
\end{array}
\right.
\]
We define $\UU_T(\RR) = (\GG \cup \GGc, Q, q^f, \sysu)$ where $Q = Q_\AA \cup Q_\BB$, $q^f = Q_\AA^f$ and
$\sys_\UU = \sysb \cup \sysa \cup \sysac \cup \sysi$.

\begin{lemma}
\label{l-basic_A+B-1}
Let $s \in \TT(\GG \cup \GGc)$. Let $q \in Q_\AA$. 
$s \to_{\sys_\UU}^+ q$ iff $s \to_{\sysa \cup \sysac}^+ q$.
\end{lemma}

\begin{proof}
$\Leftarrow$: because by definition $\sys_\UU$ contains all the rules of $\sysa \cup \sysac$.\\[.1em]
%
$\Rightarrow$: the only rules that lead to a state in $Q_\AA$ are
those in $\sysa \cup \sysac$.
\end{proof}

\begin{lemma}
\label{l-basic_A+B-2}
Let $s \in \TT(\GG \cup \GGc)$.
Let $\state{(\sto{l}{u})\theta} \in Q_\BB$.
$s \to_{\sysu}^+ \state{(\sto{l}{u})\theta}$ iff $\exists \sigma:\Var(\sto{l}{u}) \to \TT(\GG \cup \GGc)$ such that 
$s = (\sto{l}{u})\sigma$ and $\forall x \in \Var(\sto{l}{u}) \cap \Var(r)$, $x\sigma \to_{\sysa \cup \sysac}^+ x\theta$.
\end{lemma}

\begin{proof}
\hspace*{1em}{~}\\
$\Leftarrow$: $s = (\sto{l}{u})\sigma \to_{\sysa \cup \sysac}^+ (\sto{l}{u})\theta$;
we reach $\state{(\sto{l}{u})\theta}$ using matching rules of $\sysb$.\\[.1em]
$\Rightarrow$: by induction on the structure of $\sto{l}{u}$.\\
If $l/u \in \VV$, we have two cases:\\
a) $l/u \not\in \Var(r)$: then $\state{(\sto{l}{u})\theta} = \state{x}$. The sequence
$s \to_{\sysu}^+ \state{x}$ uses propagation rules only. 
We take $\sigma: \sto{l}{u} \mapsto s$ so that 
$(\sto{l}{u})\sigma = s$; the second requirement is trivially satisfied as
$\Var(\sto{l}{u}) \cap \Var(r) = \emptyset$.\\
b) $\sto{l}{u} \in \Var(r)$: then $(\sto{l}{u})\theta = q$ 
for some $q \in Q_\AA$. The last step of the sequence uses necessarily 
the interaction rule $q \to \state{q}$ 
and we may write $s \to^+_\sysu q$.
By Lemma~\ref{l-basic_A+B-1}, we get $s \to^+_{\sysa \cup \sysac} q$.
We take $\sigma: \sto{l}{u} \mapsto t$ with $t$ such that $t \to^+_\sysa q$
which is possible because by hypothesis every state of $Q_\AA$ is accessible.
We have $\sto{l}{u}\sigma = t \to^+_\sysa q = (\sto{l}{u})\theta$.\\
If $\sto{l}{u}$ is a constant,
we can only have a matching rule $s \to \state{s}$, 
$\sto{l}{u} = s$ and $\Var(l/u) = \varnothing$. We take for $\sigma$ the empty
substitution.\\
Otherwise, we may write $\sto{l}{u} = f(\sto{l}{u.1}, \ldots, \sto{l}{u.n})$
and the last step of the sequence $s \to_{\sysu}^+ \state{(\sto{l}{u})\theta}$
uses necessarily the matching
rule 
\[
f(\state{(\sto{l}{u.1})\theta}, \ldots, \state{(\sto{l}{u.n})\theta}) \to \state{(\sto{l}{u})\theta}
\] so we may write
\[
s = f(\seq{s}) \to_\sysu^+ 
f(\state{(\sto{l}{u.1})\theta}, \ldots, \state{(\sto{l}{u.n})\theta})  
\to_\sysb \state{(\sto{l}{u})\theta}
\]
The induction hypothesis yields 
$\forall i$, $1 \leq i \leq n$, 
$\exists \sigma_i: \Var(\sto{l}{u.i}) \to \TT(\GG \cup \GGc)$ such that 
$s_i = (\sto{\sto{l}{u}}{i})\sigma_i$ and 
$\forall x \in \Var(\sto{\sto{l}{u}}{i}) \cap \Var(r)$, 
$x\sigma_i \to_{\sysa \cup \sysac}^* x\theta$.
We take $\sigma = \bigcup_{i=1}^n \sigma_i$ which is possible because $l$ is linear.
Then we have  $s = f(\sto{\sto{l}{u}}{1})\sigma, \ldots, (\sto{\sto{l}{u}}{i})\sigma)$ 
and  $\forall x \in \Var(l/u) \cap \Var(r)$, 
$x\sigma \to_{\sysa \cup \sysac}^* x\theta$.
\end{proof}

\begin{corollary}
\label{c-basic_A+B}
$L(\UU_T(\RR)) = T$.
\end{corollary}

\section{Recognizability of $(\tobu^ *_\RR)[T]$}
The goal of this section is to construct an automaton which
recognizes the set $(\tobu_\RR^*)[T]$ of ground terms that $bu$-rewrite to a
term in $T$. The construction is a generalization of \cite{J96}.

The construction
starts with $\CC_T(\RR) = (\GG\cup \GGc,Q,q^f,\sys) = \UU_T(\RR)$
(constructed in Section~\ref{ss-step2}).
We saturate the transition rules $\sys$ of $\CC_T(\RR)$ under the
following inference rule:

\begin{equation}
\label{eq-saturation-bu}
\frac
{l \to r \in \RR, \quad r\theta \to_{\sys}^* q}
{\sys = \sys \cup \{ \state{l\theta} \to q\}}
%\tag{$\ast$}
\end{equation}
with $q \in Q$, $\theta$ mapping the variables in $\Var(r) \cap
\Var(l)$ to states in $Q_\AA$.
Because $Q$ is finite and no new state is added by ($\ref{eq-saturation-bu}$), the
saturation process terminates. 

\noindent
Examples:
\begin{displaymath}
\frac{
g(g(x,b),a) \to g(x,b), g(q_a,b) \to_\sys^* q^f
}
{
\sys = \sys \cup \{ \state{g(g(q_a,b),a)} \to q^f \}
}
\end{displaymath}
\begin{displaymath}
\frac{
g(g(x,b),a) \to g(x,b), g(q_a,b) \to_\sys^* 
\state{g(q_a,b)}
}
{
\sys = \sys \cup \{ \state{g(g(q_a,b),a)} \to \state{g(q_a,b)} \}
}
\end{displaymath}
No more rule can be added.
We verify that the term $g(g(g(a,b),a),a)$ which reduces to $g(a,b) \in T$ is recognized by $\CC_T(\RR)$:
\[
\begin{array}{l}
g(g(g(a,b),a),a) \to^+ g(g(g(q_a,\state{b}),\state{a}),\state{a}) \to_\sysi \\
g(g(g(\state{q_a},\state{b}),\state{a}),\state{a}) \to \\
g(g(\state{g(q_a,b)},\state{a}),\state{a}) \to\\ 
g(\state{g(g(q_a,b),a)},\state{a}) \to\\
g(\state{g(q_a,b)},\state{a}) \to \state{g(g(q_a,b),a)} \to q^f
\end{array}
\]

%% 
We now want show formally that $L(\CC_T(\RR)) = (\tobu_\RR^*)[T]$ 
upon termination. 
The technical lemmas will operate using $\toro_\RR^*$ rather than using $\tobu_\RR^*$.
But we will go back to  $\tobu_\RR$ with Definition~\ref{d-bottom-up-rewriting}.

\begin{lemma}
\label{l-aux-bottom-up-property1}
Let $s, t \in \TT(\GG \cup \GGc)$ such that $s \toro_\RR^* t$.
If $t \to_\sysu^+ q$ then $s \to_\sys^+ q$.
\end{lemma}

\begin{proof}
By induction on the length of $s \toro_\RR^* t$.\\
If the length is $0$, we have $s = t$ and the result follows from Lemmas~\ref{l-basic_A+B-1} when $q \in Q_\AA$ and from Lemma~\ref{l-basic_A+B-2} when $q \in Q_\BB$.\\
If the length is strictly greater than $0$, 
let $U = \{ u_1, \ldots, u_m \}$ be the set of minimal
occurrences in $s$ where a contraction occurs in the $\circ$-rewrite sequence $s \toro_\RR^* t$.
It follows that $s$ may be written as $s = C[s_1, s_2, \ldots, s_m]_U$.
In the rewrite sequence $s \toro_\RR^* t$, we consider the first step where a contraction
occurs at $u_1$.
We may now write
\[
\begin{array}{l}
s = C[s_1, s_2, \ldots, s_m] \stackrel{\not\leq u_1}{\toro_\RR^*} C[l\sigma, s'_2 \ldots, s'_m] \stackrel{u_1}{\toro_\RR}\\
C[r\sigma^\circ, s'_2, \ldots, s'_m] \toro_\RR^* C[t_1, t_2, \ldots, t_m] = t
\end{array}
\]
with $s_1 = f(\seq{h}) \stackrel{\neq \nopos}{\toro_\RR} l\sigma = f(\seq{l})\sigma$ for some rewrite rule $l \to r$ and 
some substitution
$\sigma:\Var(l) \to \TT(\GG \cup \GGc)$., 

Using the hypothesis $t \to_\sysu^+ q$, we may write
\[
t = C[t_1,\ldots, t_m] \to_\sysu^* C[\alpha_1, \ldots, \alpha_m] \to_\sysu^* q
\]
We have $r\sigma^\circ \toro_\RR^* t_1 \to_\sysu^+
 \alpha_1$. The induction hypothesis yields $r\sigma^\circ \to_\sys^+ \alpha_1$
which can be decomposed into $r\sigma^\circ \to_\sys^* r\theta \to_\sys^* r\theta \to_\sys^* \alpha_1$
for some substitution $\theta:\Var(l) \cap \Var(r) \to Q$.
As $\sigma^\circ$ contains only marked symbols, only marked rules of $\sysac$ can be applied in 
$r\sigma^\circ \to_\sys^* r\theta$ so we get that $r\sigma^\circ \to_\sysac^* r\theta$
with $\theta:\Var(l) \cap \Var(r) \to Q_\AA$.
Using Lemma~\ref{l-mark-to-unmark}, we get $r\sigma \to_\sysa^* r\theta$.
So 
\begin{equation}
\label{eq-l-aux-bottom-up-property1-1}
\forall x \in \Var(l) \cap \Var(r), x\sigma \to_\sysa^* x\theta
\end{equation}
% 
$\forall i$, $1 < i \leq m$, we have $s_i \toro_\RR^* t_i \to_\sysu^+ \alpha_i$, which by induction hypothesis
gives $\forall i$, $1 \leq i \leq m$, $s_i \to_\sysu^+ \alpha_i$.\\
%
From the rewrite rule $l \to r$ and the fact that $r\theta \to_\sys^* \alpha_1$,
we derive the existence of the saturation rule 
$\state{l\theta} \to \alpha_1$ in $\sys$.\\
%
By construction, $\forall j$, $1 \leq j \leq n$, $h_j \toro_\RR^* l_j\sigma$.\\
If $l_j \in \Var(r)$, from $(\ref{eq-l-aux-bottom-up-property1-1})$, we get $l_j\sigma \to_\sysa^+ l_j\theta$ 
and using an interaction rule of $\sysi$, $l_j\theta \to_\sysi \state{l_j\theta}$.\\
Otherwise, from $(\ref{eq-l-aux-bottom-up-property1-1})$ and Lemma~\ref{l-basic_A+B-2}, we get $l_j\sigma \to_\sysu^+ \state{l_j\theta}$.\\
From the two last sentences we get
\begin{displaymath}
\forall j, 1 \leq j \leq n, h_j \to_\sysu^+ \state{l_j\theta}
\end{displaymath}
Finally we write
\[
\begin{array}{l}
s = C[s_1, s_2 \ldots, s_m] \to_\sys^+  C[f(\state{l_1\theta}, \ldots, \state{l_n\theta}), \alpha_2, \ldots, \alpha_m] \to_\sysb\\
C[\state{l\theta}, \alpha_2, \ldots, \alpha_m] \to_\sys C[\alpha_1,
\alpha_2, \ldots, \alpha_m] \to_\sys^* q
\end{array}
\]
so $s \to_\sys^* q$ which ends the proof.
\end{proof}

\begin{lemma}
\label{l-bottom-up-property1}
$(\tobu_\RR^*)[T] \subseteq L(\CC_T(\RR))$.
\end{lemma}
\begin{proof}
Let $s \in \TT(\GG)$ such that $s \tobu_\RR^* t$ for some $t \in T$.
By Definition~\ref{d-bottom-up-rewriting}, $s \toro_\RR^* t'$ for some $t'$ such that $\unmar(t') = t$.
We have $t \to_\sysa^+ q^f$ for some $q^f \in Q^f_\AA = Q^f$.
It follows that $t' \to_{\sysa \cup \sysac}^+ q^f$.
Lemma~\ref{l-aux-bottom-up-property1} yields $s \to_\sys^+ q^f$ so $s \in L(\CC_T(\RR))$.
\end{proof}

\begin{lemma}
\label{l-aux-bottom-up-property2}
Let $s \in \TT(\GG \cup \GGc)$ and $q \in Q$ such that $s \to_\sys^+ q$.
\begin{enumerate}
\item
If $s \to_\sys^+ q \in Q_\AA$ then $\exists t \in \TT(\GG \cup \GGc)$ such that $s \toro_\RR^* t \to_{\sysa \cup \sysac}^+ q$
\item 
If $s \to_\sys^+ q = \state{(\sto{l}{u})\theta} \in Q_\BB$ then $\exists \sigma:\Var(\sto{l}{u}) \to \TT(\GG \cup \GGc)$ such that $s \toro_\RR^* (\sto{l}{u})\sigma$ and
$\forall x \in \Var(\sto{l}{u}) \cap \Var(r)$, $x\sigma \to_{\sysa \cup \sysac}^* x\theta$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let $\sys^k$ denote the value of $\sys$ after the $k$-th transition
rule has been added by the saturation rule 
$(\ref{eq-saturation-bu})$. We have $s \to_{\sys^k}^+ q$ for
some $k \geqslant 0$. We prove statements\emph{~1} and \emph{2} by induction on
$k$. If $k = 0$ then the result follows from Lemmas~\ref{l-basic_A+B-1} and \ref{l-basic_A+B-2}. Let
$s \to_{\sys^{k+1}}^+ q$. We use a second induction on the number of
steps which use the (unique) transition rule
$\state{l\theta} \to \alpha \in \sys^{k+1} \setminus \sys^k$. 
If this number is zero then the result
follows from the first induction hypothesis. Otherwise 
suppose this rule is created from $l \to r \in \RR$ and
$r\theta \to_{\sys^k}^* \alpha$. 
We may write
\[
s = C[s_0] \to_{\sys^k}^+ C[\state{l\theta}] \to_{\sys^{k+1}} C[\alpha]
\to_{\sys^{k+1}}^* q
\]
We will define a substitution
$\sigma:\Var(l) \to \TT(\GG \cup \GGc)$
such that
$s = C[s_0] \toro_\RR^* C[l\sigma] \toro_\RR C[r\sigma^\circ] \to_{\sys^k}^+ C[\alpha]$.
Then the second induction hypothesis applied to
$C[r\sigma^\circ] \to_{\sys^{k+1}}^+ q$ yields the desired result. \\
%
We have 
$s_0 \to_{\sys^k}^+ \state{l\theta}$.
Statement\emph{~2} of the first induction hypothesis, yields
$\exists \sigma:\Var(l) \to \TT(\GG \cup \GGc)$ such that $s_0 \toro_\RR^* l\sigma$ and
$\forall x \in \Var(l) \cap \Var(r)$, $x\sigma \to_{\sysa \cup \sysac}^+ x\theta$.\\
%
By construction, we have $r\sigma \to_{\sysa \cup \sysac}^+ r\theta$.
It follows that $r\sigma^\circ \to_{\sysa \cup \sysac}^+ r\theta$.
As we already have $r\theta \to_{\sys^k}^* \alpha$,
we get the desired constraint $r\sigma^\circ \to_{\sys^k}^* \alpha$
which completes the proof.\\
%
The induction step
is summarized in the following diagram:
\[
\xymatrix{
\stackrel{s = C[s_0]}{\circ} \ar[r] _-{\sys^k} ^-{*} \ar[d] _-{\RR} ^-{*} & C[\state{l\theta}] \ar[r] _-{\sys^{k+1}} & C[\alpha] \ar[r] _-{\sys^{k+1}} ^-{*} & q      \\
C[l\sigma]\circ \ar[r] _-{\RR}                    & C[r\sigma^\circ] \ar[r] _-{\sys^k} ^-{*}                                 & C[r\theta] \ar[u] _-{\sys^k} ^-{*}    &     \\
}
\]
\end{proof}

\begin{lemma}
\label{l-bottom-up-property2}
$L(\CC_T(\RR)) \subseteq (\tobu_\RR^*)[T]$.
\end{lemma}

\begin{proof}
Let $s \in L(\CC_T(\RR))$. We have
$s \to_\sys^+ q^f \in Q^f$.
Lemma~\ref{l-aux-bottom-up-property2} yields a term $t' \in \TT(\GG \cup \GGc)$ 
such that 
$s \toro_\RR^* t' \to_{\sysa \cup\sysac}^+ q^f$.
From Lemma~\ref{l-mark-to-unmark}, we get $t = \unmar(t') \to_\sysa^+ q^f$ so $t \in T$.
By Definition~\ref{d-bottom-up-rewriting}, we get $s \tobu_\RR^* t$.
It follows that $s \in  (\tobu_\RR^*)[T]$.
\end{proof}

\begin{corollary}
\label{c-bottom-up}
$L(\CC_T(\RR)) = (\tobu_\RR^*)[T]$.
\end{corollary}

\begin{theorem}
\label{t-bottom-up}
Bottom-up rewriting is effectively inverse recognizability preserving.
$L(\CC_T(\RR)) = (\tobu_\RR^*)[T]$.
\end{theorem}


==> strip-dependence <==
#!/bin/sh
CHAINE=$1
MOTIF="^\\\\$CHAINE\{.*\}"
shift
for i in $*
do
    egrep $MOTIF $i \
    | sed  "s/^\\\\$CHAINE{\(.*\)}/\1/" \
    | tr ['\n'] [' ']
done



